HATS-37Ab and HATS-38b: Two Transiting Hot Neptunes in the Desert

We report the discovery of two transiting Neptunes by the HATSouth survey. The planet HATS-37Ab has a mass of 0.099 +- 0.042 M_J (31.5 +- 13.4 M_earth) and a radius of 0.606 +- 0.016 R_J, and is on a P = 4.3315 days orbit around a V = 12.266 mag, 0.843 M_sun star with a radius of 0.877 R_sun. We also present evidence that the star HATS-37A has an unresolved stellar companion HATS-37B, with a photometrically estimated mass of 0.654 M_sun.The planet HATS-38b has a mass of 0.074 +- 0.011 M_J (23.5 +- 3.5 M_earth) and a radius of 0.614 +- 0.017 R_J, and is on a P = 4.3750 days orbit around a V = 12.411 mag, 0.890 M_sun star with a radius of 1.105 R_sun. Both systems appear to be old, with isochrone-based ages of 11.46 +0.79-1.45 Gyr, and 11.89 +- 0.60 Gyr, respectively. Both HATS-37Ab and HATS-38b lie in the Neptune desert and are thus examples of a population with a low occurrence rate. They are also among the lowest mass planets found from ground-based wide-field surveys to date.

==> HATS561-006_rvtable.tex <==
HATS-38 & $ 7708.80458 $ & $   -23.72 $ & $     7.70 $ & $   18.0 $ & $   10.0 $ & $   0.262 $ & HARPS \\
HATS-38 & $ 7736.74573 $ & $     9.76 $ & $     8.60 $ & $  -43.0 $ & $   13.0 $ & $   0.648 $ & FEROS \\
HATS-38 & $ 7737.84703 $ & $    -0.54 $ & $     8.20 $ & $  -17.0 $ & $   12.0 $ & $   0.900 $ & FEROS \\
HATS-38 & $ 7740.84458 $ & $    -8.94 $ & $     9.70 $ & $   38.0 $ & $   14.0 $ & $   0.585 $ & FEROS \\
HATS-38 & $ 7741.83263 $ & $    20.76 $ & $     7.90 $ & $   -7.0 $ & $   12.0 $ & $   0.811 $ & FEROS \\
HATS-38 & $ 7759.79504 $ & $    50.26 $ & $     9.00 $ & $  -29.0 $ & $   13.0 $ & $   0.917 $ & FEROS \\
HATS-38 & $ 7804.60303 $ & $    -6.22 $ & $     8.40 $ & $   -7.0 $ & $   11.0 $ & $   0.158 $ & HARPS \\
HATS-38 & $ 7805.54338 $ & $    -8.04 $ & $    10.10 $ & $   35.0 $ & $   14.0 $ & $   0.373 $ & FEROS \\
HATS-38 & $ 7805.60189 $ & $   -20.22 $ & $     6.60 $ & $  -11.0 $ & $    9.0 $ & $   0.387 $ & HARPS \\
HATS-38 & $ 7806.61869 $ & $    -1.12 $ & $     8.40 $ & $   15.0 $ & $   11.0 $ & $   0.619 $ & HARPS \\
HATS-38 & $ 7806.78686 $ & $     5.26 $ & $    12.10 $ & $    8.0 $ & $   17.0 $ & $   0.658 $ & FEROS \\
HATS-38 & $ 7807.54628 $ & $   -21.74 $ & $    13.50 $ & $  125.0 $ & $   18.0 $ & $   0.831 $ & FEROS \\
HATS-38 & $ 7829.55448 $ & $     7.86 $ & $     8.80 $ & $  -27.0 $ & $   13.0 $ & $   0.862 $ & FEROS \\
HATS-38 & $ 7830.69385 $ & $   -10.24 $ & $     8.50 $ & $   12.0 $ & $   13.0 $ & $   0.122 $ & FEROS \\
HATS-38 & $ 7848.60266 $ & $   -18.23 $ & $     3.02 $ & $   -0.5 $ & $   14.9 $ & $   0.215 $ & PFS \\
HATS-38 & $ 7849.55287 $ & $    -1.57 $ & $     3.11 $ & $   12.9 $ & $   19.6 $ & $   0.433 $ & PFS \\
HATS-38 & $ 7850.56508 $ & $     5.85 $ & $     3.02 $ & $   -3.7 $ & $   11.4 $ & $   0.664 $ & PFS \\
HATS-38 & $ 7851.62685 $ & $    11.30 $ & $     3.89 $ & $  -25.4 $ & $   40.4 $ & $   0.907 $ & PFS \\
HATS-38 & $ 7862.63029 $ & \nodata      & \nodata      & $    9.0 $ & $   10.3 $ & $   0.422 $ & PFS \\
HATS-38 & $ 7866.48140 $ & $    -6.92 $ & $     3.90 $ & $   10.0 $ & $    5.0 $ & $   0.302 $ & HARPS \\
HATS-38 & $ 7866.52106 $ & $   -14.82 $ & $     4.40 $ & $    0.0 $ & $    6.0 $ & $   0.311 $ & HARPS \\
HATS-38 & $ 7867.48250 $ & $     1.88 $ & $     5.80 $ & $    1.0 $ & $    7.0 $ & $   0.531 $ & HARPS \\
HATS-38 & $ 7867.50397 $ & $    -1.52 $ & $     6.70 $ & $   -5.0 $ & $    9.0 $ & $   0.536 $ & HARPS \\
HATS-38 & $ 7868.49777 $ & $    -6.32 $ & $     7.70 $ & $    0.0 $ & $   10.0 $ & $   0.763 $ & HARPS \\
HATS-38 & $ 7868.52092 $ & $     2.58 $ & $     7.80 $ & $   -9.0 $ & $   10.0 $ & $   0.768 $ & HARPS \\
HATS-38 & $ 7870.52143 $ & $    -1.52 $ & $     4.40 $ & $   -3.0 $ & $    6.0 $ & $   0.225 $ & HARPS \\
HATS-38 & $ 7870.54312 $ & $    -9.22 $ & $     4.40 $ & $   -1.0 $ & $    6.0 $ & $   0.230 $ & HARPS \\
HATS-38 & $ 7871.52764 $ & $     0.18 $ & $     3.90 $ & $    1.0 $ & $    5.0 $ & $   0.455 $ & HARPS \\
HATS-38 & $ 7871.54726 $ & $    -0.32 $ & $     4.40 $ & $   -3.0 $ & $    6.0 $ & $   0.460 $ & HARPS \\
HATS-38 & $ 7887.50781 $ & $   -35.12 $ & $    13.40 $ & $    5.0 $ & $   18.0 $ & $   0.108 $ & HARPS \\
HATS-38 & $ 7887.53008 $ & $   -14.52 $ & $    15.00 $ & $    5.0 $ & $   20.0 $ & $   0.113 $ & HARPS \\
HATS-38 & $ 7890.47840 $ & $    10.18 $ & $     7.80 $ & $   -4.0 $ & $   10.0 $ & $   0.787 $ & HARPS \\
HATS-38 & $ 7890.50175 $ & $     9.78 $ & $     8.40 $ & $   -1.0 $ & $   11.0 $ & $   0.792 $ & HARPS \\


==> HATS567-001_rvtable.tex <==
HATS-37 & $ 7505.50363 $ & $   -43.39 $ & $    15.00 $ & $   83.0 $ & $   19.0 $ & $   0.268 $ & HARPS \\
HATS-37 & $ 7507.79700 $ & $    32.57 $ & $    12.00 $ & $  108.0 $ & $   16.0 $ & $   0.797 $ & HARPS \\
HATS-37 & $ 7557.51991 $ & $     0.29 $ & $     2.71 $ & $   31.5 $ & $   10.7 $ & $   0.277 $ & PFS \\
HATS-37 & $ 7559.58237 $ & \nodata      & \nodata      & $   15.2 $ & $    8.4 $ & $   0.753 $ & PFS \\
HATS-37 & $ 7559.61286 $ & $    12.06 $ & $     3.25 $ & $    0.0 $ & $   11.2 $ & $   0.760 $ & PFS \\
HATS-37 & $ 7614.48266 $ & $     0.50 $ & $     4.95 $ & $   32.2 $ & $   17.6 $ & $   0.427 $ & PFS \\
HATS-37 & $ 7615.48351 $ & $     4.63 $ & $     4.11 $ & $    3.8 $ & $   10.5 $ & $   0.658 $ & PFS \\
HATS-37 & $ 7617.48123 $ & $    -5.21 $ & $     3.30 $ & $  -36.9 $ & $   10.0 $ & $   0.120 $ & PFS \\
HATS-37 & $ 7619.48263 $ & $    18.92 $ & $     7.62 $ & $ -107.5 $ & $   33.0 $ & $   0.582 $ & PFS \\
HATS-37 & $ 7622.48860 $ & $   -15.30 $ & $     3.16 $ & $   27.1 $ & $   11.4 $ & $   0.276 $ & PFS \\
HATS-37 & $ 7623.47962 $ & $    -7.39 $ & $     3.12 $ & $   10.3 $ & $   11.8 $ & $   0.504 $ & PFS \\
HATS-37 & $ 7624.49150 $ & $     6.33 $ & $     4.59 $ & $   36.5 $ & $   13.4 $ & $   0.738 $ & PFS \\
HATS-37 & $ 7849.68766 $ & $    25.22 $ & $     4.06 $ & $  -52.0 $ & $   10.3 $ & $   0.728 $ & PFS \\
HATS-37 & $ 7858.79784 $ & $    -0.39 $ & $     4.54 $ & $ -130.3 $ & $   16.1 $ & $   0.831 $ & PFS \\

